Leveraging Crowd for Game-based Learning: A Case Study of Privacy Education Game Design and Evaluation by Crowdsourcing

As the Internet grows in importance, it is vital to develop methods and techniques for educating end-users to improve their awareness of online privacy. Web-based education tools have been proven effective in many domains and have been increasingly adopted by many online professional and educational services. However, the design and development of Web-based education tools for online privacy is still in the early stage. The traditional solutions always involve privacy experts who have sophisticated expertise. Such involvement can make the tool development costly. Furthermore, it is not clear how inspiring and effective these education tools are to general users of varying backgrounds, specially to novice users who have rarely dealt with online privacy issues before. In this paper, we design, develop, and evaluate a game-based privacy learning system by leveraging the wisdom of a crowd of non-experts on Amazon Mechanic Turk. Empirical study demonstrates that the crowd can provide high-quality ideas of designing and developing a practical, educational privacy learning game.

==> summary.tex <==
\PART{B}{Project Summary}
\noindent{\bf Overview.} As the Internet grows in importance, it is vital to develop methods and techniques for educating end-users to improve their awareness of online privacy.  Web-based education tools have been proven  effective in many domains and  
have been increasingly adopted by many online professional and educational services. However, the development of Web-based education tools for online privacy is still in the early stages. Given the wide use of Internet and the severe impact of privacy accidents, there exists an urgent need for developing privacy education tools that can help to educate end-users online privacy. 

Developing effective privacy education techniques is challenging. The traditional solutions always involve privacy experts who have sophisticated expertise, deep technical skills, as well as broad experience. However, the involvement of professionals can make the tool development costly. Furthermore, it is not clear how motivating, inspiring, and/or effective these education tools are to general users of varying backgrounds, experience, and expertise of privacy, especially to novice users who have rarely dealt with privacy issues.

{\em Crowdsourcing} is an emerging paradigm that industry, government, and academia employs to harness thousands of individuals' cognitive abilities. However, the output of crowdsourcing often suffers from low quality. On the other hand, {\em groupsourcing} enables to collect information from a specific, named group that comprises of like-minded individuals. Due to the small number of participants who are of similar backgrounds, groupsoucing solutions may consist of significant bias. 
%It has shown in many domains that by allowing Web-based distributed problem solving and production, both crowdsourcing and groupsourcing can produce novel ideas that are task-appropriate and high in quality. 

\vspace{0.1in}
\noindent{\bf Intellectual merit.} 
This interdisciplinary research between a computer scientist and two social scientists aims to exploit both groupsourcing and crowdsourcing approaches to develop effective education tools of online privacy, hoping to integrate the advantages of both crowdsourcing and groupsourcing approaches while eliminating the disadvantages of two. The project aims to (1) use groupsourcing (in particular college students) for the generation of innovative ideas for the design of privacy education tools; and (2) utilize both groupsourcing and crowdsourcing as well as expert opinions for the evaluation and assessment of the developed education tools. This open collaboration of college students, experts, and crowds will facilitate the development of fun and easy to use privacy education tools that can be used by the general public.  
The project focuses on the privacy issues of three popular Internet application scenarios: social networking, cloud computing, and mobile computing. 
The theoretical significance is that the proposal will advance the field by addressing four important issues that have not been explored extensively. First, it designs novel methods based on {\em crowd-based generic algorithms} to generate collective wisdom from non-expert user groups for the development of innovative ideas of privacy education tools. Second, it investigates the main characteristics of a {\em wise} group that is capable of developing creative and high-quality ideas for privacy training. Third, it develops various methods to enhance originality and practicality of the ideas generated by the non-expert groups. 
Fourth, it integrates groupsourcing, crowdsourcing, and experts' opinions to evaluate the effectiveness of the developed privacy training tool. 
% by measuring  trainees' reaction, learning, behavior, and results of using the tool. 
%it explores various effectiveness evaluation methods and metrics to measure the quality of crowd-generated ideas and opinions. 

\vspace{0.1in}
\noindent{\bf Broad impacts.} First, as the lack of understanding about online data privacy is a global issue, providing effective training and education tools to improve the end-users' awareness of online privacy will benefit Internet users around the world. Second, if successful, the proposed approaches can dramatically reduce the overall human and financial cost of designing and developing privacy training tools. 
Third, the proposed techniques and methods will contribute to not only the computer science community but also the social science community. 
Last but not least, research results will be disseminated broadly through curricular materials appropriate for computer science, College of Arts and Letters, and MBA students. 
This interdisciplinary project is appropriate for EAGER due to its {\em high risk - high payoff}. If its hypothesis that integrating groupsourcing and crowdsourcing is suitable for developing effective privacy training techniques is correct, it will dramatically advance the research in security/privacy and social science. 

